A Neural Scaling Law from Lottery Ticket Ensembling

Neural scaling laws (NSL) refer to the phenomenon where model performance improves with scale. Sharma & Kaplan analyzed NSL using approximation theory and predict that MSE losses decay as $N^{-\alpha}$, $\alpha=4/d$, where $N$ is the number of model parameters, and $d$ is the intrinsic input dimension. Although their theory works well for some cases (e.g., ReLU networks), we surprisingly find that a simple 1D problem $y=x^2$ manifests a different scaling law ($\alpha=1$) from their predictions ($\alpha=4$). We opened the neural networks and found that the new scaling law originates from lottery ticket ensembling: a wider network on average has more "lottery tickets", which are ensembled to reduce the variance of outputs. We support the ensembling mechanism by mechanistically interpreting single neural networks, as well as studying them statistically. We attribute the $N^{-1}$ scaling law to the "central limit theorem" of lottery tickets. Finally, we discuss its potential implications for large language models and statistical physics-type theories of learning.

==> future.tex <==
{\bf Eric's suggestion: (1) relate $\beta$ to the structure of correlation matrix; (2) a toy model where you can control $\beta$; (3) detect redundancy in NN (e.g., for Pythia models). Maybe for each quanta, do a analysis similar to this (https://arxiv.org/abs/2106.03485) (4) understanding LT (estimating $\beta$) from logit distribution.}


% abstract: 
Neural scaling laws (NSL) are the observations that model performance improves with scale. Two main NSL theories, regression on data manifold (Sharma \& Kaplan) and Quantization model (Michaud et al.), are capable of predicting some empirical phenomenon while falling short for others. By studying their failure modes, we find a new mechanism of neural scaling law (NSL) from lottery tickets ensembling (LTE): Larger networks contain more lottery tickets, ensembling of which reduces losses. We demonstrate in a toy regression setup how to find "lottery tickets" by reverse engineering neural networks. %By incorporating LTE into consideration, we are able to make predictions more aligned with empirical experiments.   

Similar to statistical physics, lottery tickets can behave like particles possibly with interactions. When $N$ lottery tickets give rise to a scaling law $\ell\propto N^{-\beta}$, $\beta>1, \beta=1$ and $\beta<1$ imply that these lottery tickets have interactions similar to fermions, independent particles, and bosons, respectively. In the language of the Quanta model (Michaud et al.), quanta are independent particles, but each quantum is in turn made up of lottery tickets which could be bosonic, fermionic or independent. The augmented quantization model is able to estimate $\beta$ for language models. In particular, we find that Pythia models are strongly bosonic ($\beta\sim 0.2$), implying that there is large room for its scaling law to improve.
    From a high level, LTE suggests the role of redundancy in neural networks, which might be the key to unlock model capacity but obscure interpretability.


When $n$ lottery tickets are ensembled, the loss can decay as $n^{-\beta}$. The value of $\beta$ depends on how lottery tickets are correlated. $\beta=1$/$\beta<1$/$\beta>1$ means lottery tickets are independent, correlated or anti-correalted, anologous to three types of particles in statistical physics: independent particles, bosons and fermions. It is clear that larger $\beta$ (more fermionic) is desirable in terms of model capacity (since fewer lottery tickets are needed to reach certain performance). So, an interesting question to ask is:

\begin{center}
    \fbox{Q: Are (current) language models bosons, fermions or independent particles?}
\end{center}

To analyze language models, we need to incorporate the LTE mechanism into the Quanta model. The Quanta model suggests that the task of language modeling can be decomposed into many irreducible \textit{quanta} (subtasks). Our LTE mechanism points out, each quantum is actually reducible, possibly containing many lottery tickets, i.e., lottery tickets are the building blocks of quanta. This story is a repetition of the history of physics:  people thought that protons and neutrons are the fundamental particles, until high-energy experiments tore them apart and found even smaller particles called quarks. So we call the improved quanta model (augmented with LTE) \textit{the quark model}. The quark model is able to predict the $\beta$ value for language models. In particular, we get $\beta\sim 0.2$ for the Pythia model, which means Pythia model is strongly bosonic, implying there might be large room for optimization.

Note that we have assumed the errors of lottery tickets to be independent (orthogonal) of each other. In general, the scaling law can be $n^{-\beta}, \beta\geq 0$. If error functions are anti-correlated or correlated, the ensembling error can do better or worse than the $n^{-1}$ scaling. In the case of anti-correlation, i.e., $e_2(x) = - e_1(x)$, then two lottery tickets cancel each other's error exactly, giving rise to zero loss ($\beta=\infty$). In the case of correlation, i.e., $e_i(x)=e(x)$, ensembling cannot help reduce error at all ($\beta=0$).           

We want to borrow terminology of particle types (fermionic, bosonic, and independent particles) from statistical physics. when $\beta>1$ (lottery tickets are anti-correlated), we call they are "fermionic" (since fermions repel each other). When $\beta<1$ (lottery tickets are correlated), we call they are "bosonic" (since bosons attract each other). When $\beta=1$ (lottery tickets are independent), we call they are independent. 

\section{Generalization to the Quanta Mechanism and Beyond}

\begin{figure}[t]
    \centering
    \begin{subfigure}[]{0.45\textwidth}
\includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm]{figures/pythia_pd.pdf}
    \caption{}
    \label{fig:pythia}
    \end{subfigure}
    %\hspace{1cm}
    \begin{subfigure}[]{0.45\textwidth}
    \includegraphics[width=\linewidth, trim=0cm 0cm 0cm 0cm]{figures/pythia_pd.pdf}
    \caption{}
    \label{fig:pythia}
    \end{subfigure}
    \caption{}
    \label{fig:competition}
\end{figure}

Generalizing current quanta theory. Quanta/Subquanta

explain monogenic (large $\beta$, fermionic) vs polygenic (small $\beta$, bonsonic) based on beta value, or emergent ability

$a=0$ recovers the original quanta theory

$a$ is small, if measured by acc, good enough. So turn off gradients for already correct samples

GPT-4 and Chinchilla, (a,alpha,beta) -> alpha', predict beta value. LLMs are very bosonic, which is not good both for interpretability and for capacity.



Implication: (1) ensembling because LT not accurate, if we can get exact program, then no longer need redundancy. Both interpretability and efficiency. (2) redundancy makes interp harder. May introduce methods to reduce redundancy (but might harm performance due to less ensembling), like L1/BIMT. Justifying the validity of such interpretation methods. Only one copy of LT will remain. the squared experiment.

Futher work: (1) How to detect ensemble mechanism in LLM? Mask out some part of LLM, see if the prediction is correct. might be similar to "Redundant representations help generalization in wide neural networks" (2) So far we only study the phenomenology, but did not study the mechanism that giving rise to these phenomenology. (initial condensation?)
